Low-Shot Learning from Imaginary 3D Model

Since the advent of deep learning, neural networks have demonstrated remarkable results in many visual recognition tasks, constantly pushing the limits. However, the state-of-the-art approaches are largely unsuitable in scarce data regimes. To address this shortcoming, this paper proposes employing a 3D model, which is derived from training images. Such a model can then be used to hallucinate novel viewpoints and poses for the scarce samples of the few-shot learning scenario. A self-paced learning approach allows for the selection of a diverse set of high-quality images, which facilitates the training of a classifier. The performance of the proposed approach is showcased on the fine-grained CUB-200-2011 dataset in a few-shot setting and significantly improves our baseline accuracy.

==> sections/abstract_old.tex <==
State-of-the-art deep learning algorithms yield remarkable results in many visual recognition tasks. However, they still fail to provide satisfactory results in scarce data regimes. To a certain extent this lack of data can be compensated by multimodal information. Missing information in one modality of a single data point (e.g. an image) can be made up for in another modality (e.g. a textual description). %Here, we present new findings on few-shot learning with multi-modal data. 
Therefore, we design a few-shot learning task that is multimodal during training (i.e. image and text) and single-modal during test time (i.e. image).
In this regard, we propose a self-paced class-discriminative generative adversarial network incorporating multimodality in the context of few-shot learning. The proposed approach builds upon the idea of cross-modal data generation in order to alleviate the data sparsity problem. We improve few-shot learning accuracies on the finegrained CUB and Oxford-102 datasets.

%Firstly, we propose a novel visual recognition benchmark covering the scarce data setting. Secondly, we introduce a method for few-shot fine-grained recognition using textual descriptions of visual data, which outperforms previous approaches. Therefore we propose a self-paced learning approach 

%For each visual category, we first generate a set of images by conditioning on the textual description of the category using StackGANs. Next, we rank the generated images based on their class-discriminatory power and only pick the most discriminative images to extend the dataset. Finally, a (independent) classifier can be trained using an extended training set. %In the 1-, 2-, and 5-shot scenario the discriminative hallucinated by our method improves the top-5 accuracy by 4.9 to 8.6 percentage points on the CUB dataset.
%We find that results of our method on the CUB dataset show improved accuracy in the 1-, 2-, and 5-shot setting when employing multimodal data.

\textbf{Keywords:} Few-Shot Learning, Multimodal Learning, Meta-Learning, Fine-grained Recognition, Self-Paced Learning

==> sections/background.tex <==
\label{sec:background}

\textbf{GAN:} 
GANs \cite{goodfellow_generative_2014} consist of two adversarial agents that compete with each other during a Minimax game until reaching a Nash equilibrium at convergence of the training phase. 
Specifically, they decompose into two main components. 

First, a \emph{generator} $G$ aims to produce \emph{fake} image data $i_{fake}$ resembling \emph{real} data. That is $i_{fake} = G(z)$, given a random noise vector $z$, which induces a generator distribution $p_G$. Second, a \emph{discriminator} $D$ that defines a mapping $D: \mathcal{I}\to \left[0,1\right]$ that given an image $i\in I$, outputs a distribution w.r.t. state $s$ (i.e. \emph{fake} or \emph{real}), $p(s\mid i)=D(i)$. To this end, the GAN parameters are obtained by optimization of the loss function $\mathcal{L}\left(.\right)$,

\begin{equation}
\label{stdGANloss}
\mathcal{L}_{GAN}\left(G,D\right)=\mathbb{E}_{I}\left[\log D\left(I\right)\right]+\mathbb{E}_{z}\left[\log D\left(I,G\left(z\right)\right)\right].
\end{equation}
Specifically, training the GAN entails alternating optimization of $D$ and $G$ using stochastic gradient-based descent.
\cite{goodfellow_generative_2014} prove that a global optimium is reached when $p_g = p_{data}$, and under mild conditions  eventually $p_g$ converges to $p_{data}$.


\textbf{Conditional GAN:}
Conditional GANs (cGANs)~\cite{DBLP:journals/corr/MirzaO14} constitute an extension of the standard GAN, where the input of the generator as well as discriminator are further tied to a conditional variable containing extra information. That condition variable be an kind of auxiliary information such as a class label \cite{DBLP:journals/corr/MirzaO14}, an attribute vector \cite{yan2016attribute2image} or a semantic description~\cite{reed16_gen}. To this end, the standard loss Eq.~\ref{stdGANloss} changes slightly to

\begin{equation}
\label{cGANloss}
\mathcal{L}_{GAN}\left(G,D\right)=\mathbb{E}_{I}\left[\log D\left(I\mid y \right)\right]+\mathbb{E}_{z}\left[\log D\left(I,G\left(z\mid y\right)\right)\right],
\end{equation}
where the conditional variable is denoted as $y$. Technically, conditioning is commonly achieved by concatenation of variables, although there exist numerous possibilites - see~\cite{KwakZ16a} for some examples.
